Jointly Optimizing Preprocessing and Inference for DNN-based Visual Analytics

While deep neural networks (DNNs) are an increasingly popular way to query large corpora of data, their significant runtime remains an active area of research. As a result, researchers have proposed systems and optimizations to reduce these costs by allowing users to trade off accuracy and speed. In this work, we examine end-to-end DNN execution in visual analytics systems on modern accelerators. Through a novel measurement study, we show that the preprocessing of data (e.g., decoding, resizing) can be the bottleneck in many visual analytics systems on modern hardware. To address the bottleneck of preprocessing, we introduce two optimizations for end-to-end visual analytics systems. First, we introduce novel methods of achieving accuracy and throughput trade-offs by using natively present, low-resolution visual data. Second, we develop a runtime engine for efficient visual DNN inference. This runtime engine a) efficiently pipelines preprocessing and DNN execution for inference, b) places preprocessing operations on the CPU or GPU in a hardware- and input-aware manner, and c) efficiently manages memory and threading for high throughput execution. We implement these optimizations in a novel system, Smol, and evaluate Smol on eight visual datasets. We show that its optimizations can achieve up to 5.9x end-to-end throughput improvements at a fixed accuracy over recent work in visual analytics.

==> tex/background.tex <==
\section{Background}

We describe how DNNs are deployed in modern visual analytics systems, the full
end-to-end inference of DNNs, and advances in hardware/compilers for DNNs. In
this work, we focus on high throughput DNN inference.

\minihead{Visual analytics systems}
The majority of modern visual analytics systems we are aware of are configured
with (possibly user-defined) target DNN(s)~\cite{kang2017noscope,
anderson2018predicate, hsieh2018focus, lu2018accelerating}. Many of these modern
visual analytics systems train smaller proxy models, which we refer to as
specialized NNs, for improved performance~\cite{kang2017noscope, han2016mcdnn}.
These specialized NNs are typically used to filter irrelevant data or classify
easy examples before executing the larger, target DNN. The specialized NNs are
typically trained on a portion of the data and used in a cascade at inference
time.


\minihead{Specialization for classification}
As a case study, many systems including \noscope~\cite{kang2017noscope},
probabilistic predicates~\cite{lu2018accelerating}, and
\tahoma~\cite{anderson2018predicate}, aim to optimize visual classification.
These systems aim to reduce the cost of DNN inference by training specialized
NNs to filter inputs before executing an expensive \emph{target DNN}. \noscope
and probabilistic predicates ignores the cost of decoding video and selects
cheap specialized NNs. \tahoma considers preprocessing costs by estimating the
cost of a model by the sum of time to preprocess the input and execute the DNN
\emph{but ignores that preprocessing and DNN execution can be pipelined}. We
describe how these choices can lead to inaccurate throughput estimation for DNN
selection in \S\ref{sec:cost-model}. Furthermore, both of these systems
were implemented on older hardware (e.g., the NVIDIA P100 and K80 GPUs)
where inference is significantly slower. We show the effect of preprocessing and
modern inference hardware in these systems in \S\ref{sec:eval}.


\minihead{Specialization for approximation}
Other systems use specialized NNs as approximations to reduce invocations of the
target model. For example, the recent \blazeit system uses specialized NNs in
two ways. First, \blazeit uses specialized NNs as a control variate to reduce
the variance in sampling for aggregation queries. More accurate specialized NNs
require fewer invocations of the target model, as more accurate specialized NNs
reduces variance more. Second, \blazeit uses specialized NNs to rank frames to
invoke the target model over for \texttt{LIMIT} queries. Similarly, more
accurate specialized NNs result in better rankings, and thus fewer target model
invocations.



\begin{figure}
  \includegraphics[width=\columnwidth]{figures/e2e-diagram.pdf}
  \caption{A block diagram of end-to-end DNN inference for visual analytics
  tasks, including preprocessing and DNN execution. Much research has
  focused on optimizing DNN execution, but preprocessing can dominate execution
  times on modern hardware.}
  \label{fig:e2e-diagram}
\end{figure}

\minihead{DNN end-to-end inference}
In this work, we primarily focus on the \emph{end-to-end} inference of the DNNs
(as opposed to training). End-to-end DNN inference consists of four steps: 1)
ingesting data, 2) preprocessing the data, 3) transferring the data to the
accelerator, and 4) executing the DNN computation graph on the accelerator. We
show a diagram of this process in Figure~\ref{fig:e2e-diagram}. A large body of
research focuses on the DNN execution, but preprocessing has been relatively
neglected.

The first step of end-to-end DNN inference is ingesting the data. In visual
analytics systems, this step involves reading the compressed visual data, e.g.,
JPEG compressed image, into memory from disk or over the network. This step
typically involves high levels of branching so it is inefficient for massively
parallel arithmetic-intensive accelerators.

The second step involves decoding the compressed data, e.g., to raw pixels, and
typically applying a set of transformations over the decompressed data. For
example, the image will be resized to 224x224, converted to floating point, and
per-channel whitened for the standard ResNet-50.

The third step transfers the transformed data to the accelerator.

The fourth step executes the DNN computation graph on the accelerator and
returns the result. This step has been optimized, both in the form of more
efficient accelerators~\cite{fowers2018configurable, jouppi2017datacenter,
han2016eie} and in the form of better DNN compilers~\cite{nvidia2019tensort,
leary2017xla, pytorch2018jit}.


\minihead{Advances in hardware and compilers for DNNs}
Since deep learning has become widely adapted, accelerators for executing DNN
computation graphs have become dramatically more efficient. These new
accelerators largely rely on the fact that DNNs can be approximated with little
to no loss in accuracy~\cite{han2015deep} and that they often contain repeated
computational patterns~\cite{he2016deep}.

As a result, contemporary DNN accelerators use reduced
precision~\cite{han2015deep} and hardware units specific to DNNs, such as Tensor
Cores~\cite{markidis2018nvidia}.  For example, these are present in the NVIDIA
T4 GPU. These were not leveraged heavily in older accelerators, e.g., the NVIDIA
K80 and P100 GPUs, and can result in substantial throughput improvement in DNN
execution.

Furthermore, next generation accelerators reportedly achieve significantly
higher DNN execution throughput by further reducing precision and continuing to
specialize hardware. Next generation hardware reports up to a 2$\times$
improvement in throughput~\cite{wong2018habana}. As a result, the preprocessing
bottleneck will only grow.

These new hardware substrates are used in conjunction with new DNN compilers
that take computation graphs and emit optimized execution
plans~\cite{nvidia2019tensort, leary2017xla, pytorch2018jit}. These compilers
can efficiently use the hardware for DNN execution. As we show, this can result in
up to a 10$\times$ improvement in throughput.

